Rebuilding Factorized Information Criterion: Asymptotically Accurate Marginal Likelihood

Factorized information criterion (FIC) is a recently developed approximation technique for the marginal log-likelihood, which provides an automatic model selection framework for a few latent variable models (LVMs) with tractable inference algorithms. This paper reconsiders FIC and fills theoretical gaps of previous FIC studies. First, we reveal the core idea of FIC that allows generalization for a broader class of LVMs, including continuous LVMs, in contrast to previous FICs, which are applicable only to binary LVMs. Second, we investigate the model selection mechanism of the generalized FIC. Our analysis provides a formal justification of FIC as a model selection criterion for LVMs and also a systematic procedure for pruning redundant latent variables that have been removed heuristically in previous studies. Third, we provide an interpretation of FIC as a variational free energy and uncover a few previously-unknown their relationships. A demonstrative study on Bayesian principal component analysis is provided and numerical experiments support our theoretical results.

==> pruning.tex <==
%=======================================================
\section{Automatic Model Pruning}

A unique property of FIC is that it favors the sparse $q$. This is
because of the penalty term $-\log |\F_{\Local}|_+$.
%
%\begin{itemize}
%\item Explain why $-\log |\F_{\Local}|_+$ becomes large when
%  $\E\z_{\cdot k}\simeq \0$.
%\end{itemize}
%
This property enables to select appropriate $K$ during the
optimization. In this section, we explain how such effect occurs.

%-------------------------------------------------------
\subsection{How Does the FIC Penalty Work?}

We intuitively explain the effect $-\log |\F_{\Local}|_+$ of by using
the EM-like interpretation of the above optimization. By introducing
the posterior $p(\Z\mid \X,\EML{\Both})$ and using the Bayesian rule
that $p(A,B)/p(B|A) = p(A)$, FIC is rewritten as
%
\begin{align}
  &\max_{q}\E_q\left[
      \log \frac{p(\X,\Z\mid\EML{\Both})}{p(\Z\mid \X,\EML{\Both})}
      + \log \frac{p(\Z\mid \X,\EML{\Both})|\F_{\EML{\Both}}|^{-1/2}}{q(\Z)}
    \right]
\\
&=
  \log p(\X\mid\EML{\Both}) + \min_q \KL{q(\Z)}{\tilde{p}(\Z\mid \X,\EML{\Both})} \label{eq:KL}
\end{align}
%
where $\tilde{p}(\Z\mid \X,\EML{\Both})\propto p(\Z\mid
\X,\EML{\Both})|\F_{\EML{\Both}}|^{-1/2}$. We see that this cost
function is equivalent to that of the EM-algorithm if
$\F_{\EML{\Both}}$ is constant w.r.t. $\Z$, which tries to fit $q$ to
the posterior because of the minimization of the KL divergence. In
contrast, $\F_{\EML{\Both}}$ depends on $\Z$ in FIC, and it fits $q$ to
the skewed posterior $\tilde{p}$.
%
Figure~\ref{fig:skew} illustrates how the penalty term affects to the
true posterior. As shown, $|\F_{\EML{\Both}}|_+^{-1/2}$ has a peak
around $\z_{\cdot k}=\0$. This makes the same peak in $\tilde{p}$ in
addition to the original peak around MAP, and optimized $q$ becomes a
``sparse'' distribution, i.e., the probability of $\z_{\cdot k}=\0$ is
high.
%
\begin{figure}[tb]
  \centering
  \includegraphics[width=.9\linewidth]{skew_posterior.eps}
  \caption{The posterior, the FIC penalty, and the skewed posterior.}
  \label{fig:skew}
\end{figure}
%

%-------------------------------------------------------
By iterating the optimization of $q$, it sometimes learns $q(\z_{\cdot
  k})\simeq\delta(\z_{\cdot k}=\0)$. This means that the $k$-th
component is rarely used. Intuitively, such component has almost no
influence for modeling data, and we can eliminate it from the model,
i.e., we select the shrunken model $K-1$. Thanks to the
property of the LVMs, this strategy is justified in terms of that the
elimination improves the value of FIC.
%
\begin{proposition}\label{prop:shrink}
  Let $Q(q, K)\equiv \E_q[\log p(\X,\Z\mid\EML{\Both}, K) -
  \frac{1}{2}\log|\F_{\EML{\Local}}|] + H(q)$.  Then, if
  $q_*=\argmax_qQ(q,K)$ is the distribution that the probability of
  $\z_{\cdot k}=\0$ is one, i.e., $q_*(\Z)=q_*(\Z_{\quot
    k})\delta(\z_{\cdot k}=\0)$, then
%
  \begin{align}
    Q(q_*(\Z), \Both, K) \leq Q(q_*(\Z_{\quot k}), \{\Global,\Local_{\quot k}\}, K-1)
  \end{align}
%
  where $\Local_{\quot
    k}=\{\local_1,\dots,\local_{k-1},\local_{k+1},\dots,\local_{K}\}$
  is truncated parameters.
\end{proposition}
%
\begin{proof}[Sketch]
To prove Proposition~\ref{prop:shrink}, we use
\ref{asm:switch} that makes the marginalization of
$\local_k$ having no effect (since the $k$-th component is never
used.) 
\end{proof}
%Proposition~\ref{prop:shrink} tells us that Algorithm~(?) increases
%the marginal log-likelihood monotonically.




\subsection{Algorithm}

As explained, ``pruning'' redundant components also increases FIC as
well as the optimization w.r.t. $q$ and $\Both$. As a natural idea,
we include the model pruning operation during the optimization, which
leads Algorithm~\ref{alg:ems}.
%
\begin{algorithm}[tb]
   \caption{EMS algorithm}
   \label{alg:ems}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $\X$, maximum \#components $K_{\max}$, threshold $\delta$
   \STATE $K \gets K_{\max}$
   \REPEAT
   \STATE $q\gets \argmax_q Q(q,\Both, K)$
   \STATE $\Both\gets \argmax_\Both \E_q[\log p(\X,\Z\mid\Both, K)]$
   \IF{$\sum_n \E_q[z_{nk}]/N < \delta$}
   \STATE $K\gets K-1$ and delete the $k$-th component.
   \ENDIF
   \UNTIL{Convergence}
\end{algorithmic}
\end{algorithm}
%
This EM-like algorithm is a block coordinate ascent; each step
monotonically increases FIC and it stops at a critical point of $Q$.
%
\begin{itemize}
\item Thresholding by $\delta$ is arbitrary. This part may replace by
  the model selection via log-likelihood ratio test.
\end{itemize}

A nice property of FIC is that it does not need to compute for all
$\mathcal{K}$; the model pruning mechanism enables one-pass learning.

In addition, start from sufficiently large $K_{\max}$ may efficiently
avoid local minima.
\begin{itemize}
\item need more explanation and investigation.
\end{itemize}

%This algorithm also can be seen as a survival-of-the-fittest process:
%\begin{itemize}
%\item In initialization phase, we prepare sufficiently large $K_{\max}$
%  components that is over-representing of the model.
%\item May efficiently avoid local minima.
%\end{itemize}


%-------------------------------------------------------
\subsection{Case Study: Gaussian Mixture}

We investigate the behavior of FIC and the FAB algorithm by using a
simple example. We consider a two-components $1$-D Gaussian mixture
with unit variance:
%
\begin{align}
  p(x_n, z_n\mid\Both)=N(x_n\mid \mu_1,1)^{z_n}N(x_n\mid
  \mu_2,1)^{1-z_n} \Bern(z_n\mid\pi).
\end{align}
%
To eliminate uncertainty of data, we consider FIC expected by the data
distribution $p(x\mid\model_*)= \pi_*N(x\mid 0, 1) + (1-\pi_*)N(x\mid
1,1)$, i.e., $\E_*[\FIC{}] =$
%
\begin{align*}
  &  -\frac{N}{2}\left(\tau\E_*[(x-\EML{\mu}_1)^2] + (1-\tau)\E_*[(x-\EML{\mu}_2)^2]\right)
\\
 & + N\left(\tau\log\EML{\pi} + (1-\tau)\log(1-\EML{\pi})\right) + H(q)
\\
 & - \frac{1}{2}\left(\E_q[\log_+ N\tau] + \E_q[\log_+ N(1-\tau)]\right) + \const
\end{align*}
%
where $\tau=\sum_n\E_qz_n / N$ and $\log_+(x)=\log(x)$ if $x>1$
otherwise $\log_+(x)=0$. We see that, thanks to the expectation
$\E_*[\cdot]=\int \cdot p(x\mid\model_*)\d x$, we only need to deal
with $q$ of $\tau$, the sum of $z_n$, instead of that of the
individual $z_n$. The maximization w.r.t. $q(z_n)$ without the FIC
penalty yields the posterior $p(z_n\mid \model_*) =
\Bern(z_n\mid\omega)$~\cite{prml} where $\omega =
\EML{\pi}\Gauss_*(\EML{\mu}_1) / (\EML{\pi}\Gauss_*(\EML{\mu}_1) +
(1-\EML{\pi})\Gauss_*(\EML{\mu}_2))$ and
$\Gauss_*(\mu)=\exp(-\E_*[(x-\mu)^2]/2)/\sqrt{2\pi}$, and $\tau$
follows the Binomial distribution $q(N\tau = n)={N \choose n}\,
\omega^n (1-\omega)^{N-n}$.
%With the FIC penalty, since there is no
%closed-form solution for $q(\z)$, we directly consider $q(N\tau)$ as
%the Beta-Binomial distribution, which is more flexible than the
%Binomial. ${N \choose n}\,B(n+\alpha, N-n+\beta)/B(\alpha,\beta)$
%where
%$B(\alpha,\beta)=\Gamma(\alpha)\Gamma(\beta)/\Gamma(\alpha+\beta)$ and
%$\Gamma(\cdot)$ is the Gamma function. 
%

%%%
\begin{figure}[tb]
  \centering
  \includegraphics[width=.9\linewidth]{ptilde.eps}
  \caption{The posterior, the FIC penalty, and the skewed posterior of the GMM with $N=15$.}
  \label{fig:gmm-posteriors}
\end{figure}
%
Figure~\ref{fig:gmm-posteriors} shows the posterior, the (normalized)
FIC penalty, and the skewed posterior, which we numerically
compute. We see that the penalty has two peaks around $\tau=0$ and
$1$, and it changes the shape of the posterior that shifts the mean to
the borders. $N$, the number of samples, affects the shape of the
penalty; as $N$ increasing, the peak becomes sharper. As a result, for
larger $N$, the posterior is almost not skewed when $\omega$ is not
close to the borders, but is heavily skewed when $\omega$ is close to
the borders.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "fabcont.tex"
%%% End:

